TorchBench: Benchmarking PyTorch with High API Surface Coverage

Deep learning (DL) has been a revolutionary technique in various domains. To facilitate the model development and deployment, many deep learning frameworks are proposed, among which PyTorch is one of the most popular solutions. The performance of ecosystem around PyTorch is critically important, which saves the costs of training models and reduces the response time of model inferences. In this paper, we propose TorchBench, a novel benchmark suite to study the performance of PyTorch software stack. Unlike existing benchmark suites, TorchBench encloses many representative models, covering a large PyTorch API surface. TorchBench is able to comprehensively characterize the performance of the PyTorch software stack, guiding the performance optimization across models, PyTorch framework, and GPU libraries. We show two practical use cases of TorchBench. (1) We profile TorchBench to identify GPU performance inefficiencies in PyTorch. We are able to optimize many performance bugs and upstream patches to the official PyTorch repository. (2) We integrate TorchBench into PyTorch continuous integration system. We are able to identify performance regression in multiple daily code checkins to prevent PyTorch repository from introducing performance bugs. TorchBench is open source and keeps evolving.

==> code_cudnn.tex <==
%auto-ignore
\begin{figure}[tp]
\begin{lstlisting}[label=lst:cudnn_compare, escapechar=|, caption={An example to illustrate failed fastest CUDA kernel selection for cuDNN8.5.0. },linebackgroundcolor={
}
]
    input_shape = [1, 1024, 50, 75]
    weight_shape = (1024, 1024, 3, 3)
    weight = torch.ones(weight_shape, dtype=torch.float32, device='cuda')
    x = torch.ones(input_shape, dtype=torch.float32, device='cuda')
    bias = torch.ones((1024, ), dtype=torch.float32, device='cuda')
    F.conv2d(x, weight, bias, (1, 1), (1, 1), (1, 1), 1)
\end{lstlisting}
\end{figure}

==> code_hf_bigbird.tex <==
%auto-ignore
\begin{figure}[tp]
\begin{lstlisting}[label=lst:hf-bigbird, escapechar=|, caption={Model hf\_BigBird calls the function \texttt{numpy.random.permutation()} to generate permutations for a subset of \texttt{middle\_seq}.},linebackgroundcolor={
    \ifnum\value{lstnumber}=12
            \color{blue!10}
    \fi
}
]
def _bigbird_block_rand_mask(
        from_seq_length, to_seq_length, from_block_size, to_block_size, num_rand_blocks, last_idx=-1
    ):
    rand_attn = np.zeros((from_seq_length // from_block_size - 2, num_rand_blocks), dtype=np.int32)
    middle_seq = np.arange(1, to_seq_length // to_block_size - 1, dtype=np.int32)
    r = num_rand_blocks
    ...
    for i in range(1, from_seq_length // from_block_size - 1):
        start = i - 2
        end = i
        ...
        rand_attn[i - 1, :] = np.random.permutation(middle_seq[:start])[:r]
        ...
    return rand_attn
\end{lstlisting}
\end{figure}

==> code_single_tensor.tex <==
%auto-ignore
\begin{figure}[tp]
\begin{lstlisting}[label=lst:single_tensor, escapechar=|, caption={PyTorch uses single tensor adam optimizer by default, which triggers many tiny GPU kernels.},linebackgroundcolor={
    \ifnum\value{lstnumber}<7
    \ifnum\value{lstnumber}>4
            \color{blue!10}
    \fi
    \fi
}]        
def adam(params: List[Tensor],...
        foreach: bool = None,
        ...):
    if foreach is None:
 -      foreach = False
 +      foreach = True
    if foreach and not torch.jit.is_scripting():
        func = _multi_tensor_adam
    else:
        func = _single_tensor_adam
\end{lstlisting}
\end{figure}

==> table_all_inefficiencies.tex <==
%auto-ignore
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\footnotesize
\caption{Inefficiency patterns due to GPU idleness and overhead across different components of PyTorch software stack. PyTorch is the PyTorch core library; CUDA is the vendor library; Model means different models developed for specific tasks.}
\label{table:all_inefficiencies}
\setlength{\tabcolsep}{1pt}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|cc|cc|}
\hline
\multirow{2}{*}{Function}                          & \multirow{2}{*}{Pattern}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Related Components in\\PyTorch Software Stack\end{tabular}} & \multicolumn{2}{c|}{Symptom}                     & \multicolumn{2}{c|}{Mode}                    \\ \cline{4-7} 
                                                   &                           &                                                                                                          & \multicolumn{1}{c|}{GPU Idleness} & GPU Overhead & \multicolumn{1}{c|}{Training}   & Inference  \\ \hline
Optimizer: \_single\_tensor\_adam/sgd              & Tiny CUDA Kernels         & PyTorch, CUDA                                                                                            & \multicolumn{1}{c|}{↑}            & ↑            & \multicolumn{1}{c|}{\checkmark} &            \\ \hline
Optimizer: zero\_grad                              & Tiny CUDA Kernels         & PyTorch, CUDA                                                                                            & \multicolumn{1}{c|}{↑}            & ↑            & \multicolumn{1}{c|}{\checkmark} &            \\ \hline
Aten APIs                                          & Tiny CUDA Kernels         & PyTorch, CUDA                                                                                            & \multicolumn{1}{c|}{↑}            & ↑            & \multicolumn{1}{c|}{\checkmark} & \checkmark \\ \hline
Detectron2: post\_process                          & Tiny CUDA Kernels         & Model, CUDA                                                                                              & \multicolumn{1}{c|}{↑}            & ↑            & \multicolumn{1}{c|}{}           & \checkmark \\ \hline
Detectron2: process\_polygons                      & CPU Overloading           & Model, CUDA                                                                                              & \multicolumn{1}{c|}{↑}            & ↓            & \multicolumn{1}{c|}{\checkmark} & \checkmark \\ \hline
Detectron2: batched\_nms\_vanilla                  & CPU Overloading           & Model, CUDA                                                                                              & \multicolumn{1}{c|}{↑}            & ↓            & \multicolumn{1}{c|}{\checkmark} & \checkmark \\ \hline
Huggingface: torch.item                            & Data Movement, API misuse & Model, PyTorch                                                                                           & \multicolumn{1}{c|}{↓}            & ↑            & \multicolumn{1}{c|}{\checkmark} & \checkmark \\ \hline
Huggingface: bigbird, \_bigbird\_block\_rand\_mask & CPU Overloading           & Model, CUDA                                                                                              & \multicolumn{1}{c|}{↑}            & ↓            & \multicolumn{1}{c|}{\checkmark} &            \\ \hline
Detectron2: fasterrcnn, conv2d-relu combination    & Tiny CUDA Kernels         & Model, PyTorch                                                                                           & \multicolumn{1}{c|}{↑}            & ↑            & \multicolumn{1}{c|}{\checkmark} & \checkmark \\ \hline
Huggingface: reformer, torch.rsqrt                 & Data Movement, API misuse & Model, PyTorch                                                                                           & \multicolumn{1}{c|}{↓}            & ↑            & \multicolumn{1}{c|}{\checkmark} & \checkmark \\ \hline
LearningToPaint: cuda memcpy                       & Data Movement             & Model, CUDA                                                                                              & \multicolumn{1}{c|}{↓}            & ↑            & \multicolumn{1}{c|}{\checkmark} & \checkmark \\ \hline
\end{tabular}


\end{table*}

==> table_all_issues_backup.tex <==
%auto-ignore
\begin{table}[t]
\caption{10 issues found in PyTorch development by \tool{} in the last two years. }
\label{table:all_issues}
\centering


\begin{tabular}{|l|c|}
\hline
\multicolumn{1}{|c|}{Issue Description}                                                                                                                               & Category                \\ \hline
The nightly build script generates release based on wrong commits.                                                                                                    & Correctness             \\ \hline
\begin{tabular}[c]{@{}l@{}}Using FindCUDAToolkit in CMake causes runtime errors in some \\ environments and increase the released wheel file size a lot.\end{tabular} & Correctness             \\ \hline
TorchVision has compatibility issue for FFMPEG.                                                                                                                       & Correctness             \\ \hline
The cuBLAS workspace API changes causes potential OOM errors.                                                                                                         & Memory Issue            \\ \hline
The commit performs a duplicate error check that accesses all items in the tensors                                                                                    & Performance Degradation \\ \hline
JIT compiler has worse performance on NVIDIA M60.                                                                                                                     & Performance Degradation \\ \hline
The cuBLAS workspace size is not set to the optimal value.                                                                                                            & Performance Degradation \\ \hline
Extra out of bound checks causes performance degradations.                                                                                                            & Performance Degradation \\ \hline
Extra checks for using oneDNN causes performance degradations.                                                                                                        & Performance Degradation \\ \hline
The c10 error check template causes the performance degradations.                                                                                                     & Performance Degradation \\ \hline
\end{tabular}
\end{table}

==> table_all_models.tex <==
%auto-ignore
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\label{table:all_models}
\scriptsize
\begin{tabular}{|c|c|c|}
\hline
Domain                                   & Sub-Domain                               & Model                                  \\ \hline
\multirow{47}{*}{COMPUTER\_VISION}       & \multirow{20}{*}{CLASSIFICATION}         & alexnet                                \\ \cline{3-3} 
                                         &                                          & densenet121                            \\ \cline{3-3} 
                                         &                                          & mnasnet1\_0                            \\ \cline{3-3} 
                                         &                                          & mobilenet\_v2                          \\ \cline{3-3} 
                                         &                                          & mobilenet\_v2\_quantized\_qat          \\ \cline{3-3} 
                                         &                                          & mobilenet\_v3\_large                   \\ \cline{3-3} 
                                         &                                          & phlippe\_densenet                      \\ \cline{3-3} 
                                         &                                          & phlippe\_resnet                        \\ \cline{3-3} 
                                         &                                          & resnet152                              \\ \cline{3-3} 
                                         &                                          & resnet18                               \\ \cline{3-3} 
                                         &                                          & resnet50                               \\ \cline{3-3} 
                                         &                                          & resnet50\_quantized\_qat               \\ \cline{3-3} 
                                         &                                          & resnext50\_32x4d                       \\ \cline{3-3} 
                                         &                                          & shufflenet\_v2\_x1\_0                  \\ \cline{3-3} 
                                         &                                          & squeezenet1\_1                         \\ \cline{3-3} 
                                         &                                          & timm\_efficientnet                     \\ \cline{3-3} 
                                         &                                          & timm\_nfnet                            \\ \cline{3-3} 
                                         &                                          & timm\_regnet                           \\ \cline{3-3} 
                                         &                                          & timm\_resnest                          \\ \cline{3-3} 
                                         &                                          & vgg16                                  \\ \cline{2-3} 
                                         & \multirow{12}{*}{DETECTION}              & detectron2\_fasterrcnn\_r\_101\_c4     \\ \cline{3-3} 
                                         &                                          & detectron2\_fasterrcnn\_r\_101\_dc5    \\ \cline{3-3} 
                                         &                                          & detectron2\_fasterrcnn\_r\_101\_fpn    \\ \cline{3-3} 
                                         &                                          & detectron2\_fasterrcnn\_r\_50\_c4      \\ \cline{3-3} 
                                         &                                          & detectron2\_fasterrcnn\_r\_50\_dc5     \\ \cline{3-3} 
                                         &                                          & detectron2\_fasterrcnn\_r\_50\_fpn     \\ \cline{3-3} 
                                         &                                          & detectron2\_maskrcnn                   \\ \cline{3-3} 
                                         &                                          & doctr\_det\_predictor                  \\ \cline{3-3} 
                                         &                                          & doctr\_reco\_predictor                 \\ \cline{3-3} 
                                         &                                          & timm\_efficientdet                     \\ \cline{3-3} 
                                         &                                          & timm\_vovnet                           \\ \cline{3-3} 
                                         &                                          & vision\_maskrcnn                       \\ \cline{2-3} 
                                         & \multirow{6}{*}{GENERATION}              & DALLE2\_pytorch                        \\ \cline{3-3} 
                                         &                                          & dcgan                                  \\ \cline{3-3} 
                                         &                                          & pytorch\_CycleGAN\_and\_pix2pix        \\ \cline{3-3} 
                                         &                                          & pytorch\_stargan                       \\ \cline{3-3} 
                                         &                                          & timm\_vision\_transformer              \\ \cline{3-3} 
                                         &                                          & timm\_vision\_transformer\_large       \\ \cline{2-3} 
                                         & \multirow{2}{*}{OTHER\_COMPUTER\_VISION} & Background\_Matting                    \\ \cline{3-3} 
                                         &                                          & Super\_SloMo                           \\ \cline{2-3} 
                                         & \multirow{7}{*}{SEGMENTATION}            & detectron2\_fcos\_r\_50\_fpn           \\ \cline{3-3} 
                                         &                                          & detectron2\_maskrcnn\_r\_101\_c4       \\ \cline{3-3} 
                                         &                                          & detectron2\_maskrcnn\_r\_101\_fpn      \\ \cline{3-3} 
                                         &                                          & detectron2\_maskrcnn\_r\_50\_c4        \\ \cline{3-3} 
                                         &                                          & detectron2\_maskrcnn\_r\_50\_fpn       \\ \cline{3-3} 
                                         &                                          & pytorch\_unet                          \\ \cline{3-3} 
                                         &                                          & yolov3                                 \\ \hline
\multirow{17}{*}{NLP}                    & \multirow{15}{*}{LANGUAGE\_MODELING}     & BERT\_pytorch                          \\ \cline{3-3} 
                                         &                                          & fambench\_xlmr                         \\ \cline{3-3} 
                                         &                                          & hf\_Albert                             \\ \cline{3-3} 
                                         &                                          & hf\_Bart                               \\ \cline{3-3} 
                                         &                                          & hf\_Bert                               \\ \cline{3-3} 
                                         &                                          & hf\_Bert\_large                        \\ \cline{3-3} 
                                         &                                          & hf\_BigBird                            \\ \cline{3-3} 
                                         &                                          & hf\_DistilBert                         \\ \cline{3-3} 
                                         &                                          & hf\_GPT2                               \\ \cline{3-3} 
                                         &                                          & hf\_GPT2\_large                        \\ \cline{3-3} 
                                         &                                          & hf\_Longformer                         \\ \cline{3-3} 
                                         &                                          & hf\_Reformer                           \\ \cline{3-3} 
                                         &                                          & hf\_T5                                 \\ \cline{3-3} 
                                         &                                          & hf\_T5\_base                           \\ \cline{3-3} 
                                         &                                          & hf\_T5\_large                          \\ \cline{2-3} 
                                         & OTHER\_NLP                               & fastNLP\_Bert                          \\ \cline{2-3} 
                                         & TRANSLATION                              & attention\_is\_all\_you\_need\_pytorch \\ \hline
\multirow{2}{*}{RECOMMENDATION}          & \multirow{2}{*}{-}                       & dlrm                                   \\ \cline{3-3} 
                                         &                                          & nvidia\_deeprecommender                \\ \hline
\multirow{3}{*}{REINFORCEMENT\_LEARNING} & \multirow{3}{*}{-}                       & drq                                    \\ \cline{3-3} 
                                         &                                          & LearningToPaint                        \\ \cline{3-3} 
                                         &                                          & soft\_actor\_critic                    \\ \hline
\multirow{3}{*}{Speech}                  & RECOGNITION                              & speech\_transformer                    \\ \cline{2-3} 
                                         & \multirow{2}{*}{SYNTHESIS}               & tacotron2                              \\ \cline{3-3} 
                                         &                                          & tts\_angular                           \\ \hline
\multirow{12}{*}{Other Task}             & \multirow{12}{*}{-}                      & demucs                                 \\ \cline{3-3} 
                                         &                                          & functorch\_dp\_cifar10                 \\ \cline{3-3} 
                                         &                                          & functorch\_maml\_omniglot              \\ \cline{3-3} 
                                         &                                          & lennard\_jones                         \\ \cline{3-3} 
                                         &                                          & maml                                   \\ \cline{3-3} 
                                         &                                          & maml\_omniglot                         \\ \cline{3-3} 
                                         &                                          & moco                                   \\ \cline{3-3} 
                                         &                                          & opacus\_cifar10                        \\ \cline{3-3} 
                                         &                                          & pyhpc\_equation\_of\_state             \\ \cline{3-3} 
                                         &                                          & pyhpc\_isoneutral\_mixing              \\ \cline{3-3} 
                                         &                                          & pyhpc\_turbulent\_kinetic\_energy      \\ \cline{3-3} 
                                         &                                          & pytorch\_struct                        \\ \hline
\end{tabular}
\end{table}

==> table_all_models_2.tex <==
%auto-ignore
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{why we choose these models? even in . 84 benchmark models of 5 domains are included in \tool{}. Yueming @TODO: double check all categories such as Other. }
\label{table:all_models_2}
\centering

\begin{tabular}{|c|c|cc|}
\hline
Domain                                  & Task                         & \multicolumn{2}{c|}{Model}                                                                 \\ \hline
\multirow{24}{*}{Computer Vision}       & \multirow{10}{*}{Classification}   & \multicolumn{1}{c|}{alexnet}                                & resnet50                     \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{densenet121}                            & resnet50\_quantized\_qat     \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{mnasnet1\_0}                            & resnext50\_32x4d             \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{mobilenet\_v2}                          & shufflenet\_v2\_x1\_0        \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{mobilenet\_v2\_quantized\_qat}          & squeezenet1\_1               \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{mobilenet\_v3\_large}                   & timm\_efficientnet           \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{phlippe\_densenet}                      & timm\_nfnet                  \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{phlippe\_resnet}                        & timm\_regnet                 \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{resnet152}                              & timm\_resnest                \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{resnet18}                               & vgg16                        \\ \cline{2-4} 
                                        & \multirow{6}{*}{Detection}         & \multicolumn{1}{c|}{detectron2\_fasterrcnn\_r\_101\_c4}     & detectron2\_maskrcnn         \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{detectron2\_fasterrcnn\_r\_101\_dc5}    & doctr\_det\_predictor        \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{detectron2\_fasterrcnn\_r\_101\_fpn}    & doctr\_reco\_predictor       \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{detectron2\_fasterrcnn\_r\_50\_c4}      & timm\_efficientdet           \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{detectron2\_fasterrcnn\_r\_50\_dc5}     & timm\_vovnet                 \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{detectron2\_fasterrcnn\_r\_50\_fpn}     & vision\_maskrcnn             \\ \cline{2-4} 
                                        & \multirow{3}{*}{Generation}        & \multicolumn{1}{c|}{timm\_vision\_transformer\_large}       & pytorch\_stargan             \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{timm\_vision\_transformer}              & dcgan                        \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{pytorch\_CycleGAN\_and\_pix2pix}        & DALLE2\_pytorch              \\ \cline{2-4} 
                                        & \multirow{4}{*}{Segmentation}      & \multicolumn{1}{c|}{detectron2\_maskrcnn\_r\_101\_c4}       & detectron2\_fcos\_r\_50\_fpn \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{detectron2\_maskrcnn\_r\_101\_fpn}      & pytorch\_unet                \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{detectron2\_maskrcnn\_r\_50\_c4}        & yolov3                       \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{detectron2\_maskrcnn\_r\_50\_fpn}       &                              \\ \cline{2-4} 
                                        & Other                              & \multicolumn{1}{c|}{Background\_Matting}                    & Super\_SloMo                 \\ \hline
\multirow{10}{*}{NLP}                   & \multirow{8}{*}{Language Modeling} & \multicolumn{1}{c|}{BERT\_pytorch}                          & hf\_GPT2                     \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{fambench\_xlmr}                         & hf\_GPT2\_large              \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{hf\_Albert}                             & hf\_Longformer               \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{hf\_Bart}                               & hf\_Reformer                 \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{hf\_Bert}                               & hf\_T5                       \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{hf\_Bert\_large}                        & hf\_T5\_base                 \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{hf\_BigBird}                            & hf\_T5\_large                \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{hf\_DistilBert}                         &                              \\ \cline{2-4} 
                                        & Translation                        & \multicolumn{1}{c|}{attention\_is\_all\_you\_need\_pytorch} &                              \\ \cline{2-4} 
                                        & Other                              & \multicolumn{1}{c|}{fastNLP\_Bert}                          &                              \\ \hline
Recommendation                          & -                                  & \multicolumn{1}{c|}{nvidia\_deeprecommender}                & dlrm                         \\ \hline
\multirow{2}{*}{Reinforcement Learning} & \multirow{2}{*}{-}                 & \multicolumn{1}{c|}{drq}                                    & soft\_actor\_critic          \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{LearningToPaint}                        &                              \\ \hline
\multirow{2}{*}{Speech}                 & Recognition                        & \multicolumn{1}{c|}{speech\_transformer}                    &                              \\ \cline{2-4} 
                                        & Synthesis                          & \multicolumn{1}{c|}{tacotron2}                              & tts\_angular                 \\ \hline
\multirow{6}{*}{Other}                  & \multirow{6}{*}{-}                 & \multicolumn{1}{c|}{demucs}                                 & moco                         \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{functorch\_dp\_cifar10}                 & opacus\_cifar10              \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{functorch\_maml\_omniglot}              & pyhpc\_equation\_of\_state   \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{lennard\_jones}                         & pyhpc\_isoneutral\_mixing    \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{pyhpc\_turbulent\_kinetic\_energy}      & maml                         \\ \cline{3-4} 
                                        &                                    & \multicolumn{1}{c|}{maml\_omniglot}                         & pytorch\_struct              \\ \hline
\end{tabular}
\end{table*}

==> table_all_models_3.tex <==
%auto-ignore
\begin{table*}[]
\caption{\tool{} consists of 84 models from various domains to benchmark PyTorch.}
\label{table:all_models_3}
\centering

\begin{tabular}{llll}
\hline
Domain                                  & Task                                   & \multicolumn{2}{l}{Model}                                             \\ \hline
\multirow{26}{*}{Computer Vision}       & \multirow{11}{*}{Image Classification} & alexnet                                & resnet50                     \\ \cdashline{3-4} 
                                        &                                        & densenet121                            & resnet50\_quantized\_qat     \\ \cdashline{3-4} 
                                        &                                        & mnasnet1\_0                            & resnext50\_32x4d             \\ \cdashline{3-4} 
                                        &                                        & mobilenet\_v2                          & shufflenet\_v2\_x1\_0        \\ \cdashline{3-4} 
                                        &                                        & mobilenet\_v2\_quantized\_qat          & squeezenet1\_1               \\ \cdashline{3-4} 
                                        &                                        & mobilenet\_v3\_large                   & timm\_efficientnet           \\ \cdashline{3-4} 
                                        &                                        & phlippe\_densenet                      & timm\_nfnet                  \\ \cdashline{3-4} 
                                        &                                        & phlippe\_resnet                        & timm\_regnet                 \\ \cdashline{3-4} 
                                        &                                        & resnet152                              & timm\_resnest                \\ \cdashline{3-4} 
                                        &                                        & resnet18                               & vgg16                        \\ \cdashline{3-4} 
                                        &                                        & opacus\_cifar10                        &                              \\ \cdashline{2-4} 
                                        & \multirow{6}{*}{Object Detection}      & detectron2\_fasterrcnn\_r\_101\_c4     & detectron2\_maskrcnn         \\ \cdashline{3-4} 
                                        &                                        & detectron2\_fasterrcnn\_r\_101\_dc5    & doctr\_det\_predictor        \\ \cdashline{3-4} 
                                        &                                        & detectron2\_fasterrcnn\_r\_101\_fpn    & doctr\_reco\_predictor       \\ \cdashline{3-4} 
                                        &                                        & detectron2\_fasterrcnn\_r\_50\_c4      & timm\_efficientdet           \\ \cdashline{3-4} 
                                        &                                        & detectron2\_fasterrcnn\_r\_50\_dc5     & timm\_vovnet                 \\ \cdashline{3-4} 
                                        &                                        & detectron2\_fasterrcnn\_r\_50\_fpn     & vision\_maskrcnn             \\ \cdashline{2-4} 
                                        & \multirow{3}{*}{Image Generation}      & timm\_vision\_transformer\_large       & pytorch\_stargan             \\ \cdashline{3-4} 
                                        &                                        & timm\_vision\_transformer              & dcgan                        \\ \cdashline{3-4} 
                                        &                                        & pytorch\_CycleGAN\_and\_pix2pix        & DALLE2\_pytorch              \\ \cdashline{2-4} 
                                        & \multirow{4}{*}{Image Segmentation}    & detectron2\_maskrcnn\_r\_101\_c4       & detectron2\_fcos\_r\_50\_fpn \\ \cdashline{3-4} 
                                        &                                        & detectron2\_maskrcnn\_r\_101\_fpn      & pytorch\_unet                \\ \cdashline{3-4} 
                                        &                                        & detectron2\_maskrcnn\_r\_50\_c4        & yolov3                       \\ \cdashline{3-4} 
                                        &                                        & detectron2\_maskrcnn\_r\_50\_fpn       &                              \\ \cdashline{2-4} 
                                        & Pattern Recognition                    & Background\_Matting                    &                              \\ \cdashline{2-4} 
                                        & Video Interpolation                    & Super\_SloMo                           &                              \\ \hline
\multirow{10}{*}{NLP}                   & \multirow{8}{*}{Language Modeling}     & BERT\_pytorch                          & hf\_GPT2                     \\ \cdashline{3-4} 
                                        &                                        & fambench\_xlmr                         & hf\_GPT2\_large              \\ \cdashline{3-4} 
                                        &                                        & hf\_Albert                             & hf\_Longformer               \\ \cdashline{3-4} 
                                        &                                        & hf\_Bart                               & hf\_Reformer                 \\ \cdashline{3-4} 
                                        &                                        & hf\_Bert                               & hf\_T5                       \\ \cdashline{3-4} 
                                        &                                        & hf\_Bert\_large                        & hf\_T5\_base                 \\ \cdashline{3-4} 
                                        &                                        & hf\_BigBird                            & hf\_T5\_large                \\ \cdashline{3-4} 
                                        &                                        & hf\_DistilBert                         &                              \\ \cdashline{2-4} 
                                        & Translation                            & attention\_is\_all\_you\_need\_pytorch &                              \\ \cdashline{2-4} 
                                        & Other                                  & fastNLP\_Bert                          &                              \\ \hline
Recommendation                          & -                                      & nvidia\_deeprecommender                & dlrm                         \\ \hline
\multirow{2}{*}{Reinforcement Learning} & \multirow{2}{*}{-}                     & drq                                    & soft\_actor\_critic          \\ \cdashline{3-4} 
                                        &                                        & LearningToPaint                        &                              \\ \hline
\multirow{3}{*}{Speech}                 & Recognition                            & speech\_transformer                    &                              \\ \cdashline{2-4} 
                                        & Audio Source Separation                & demucs                                 &                              \\ \cdashline{2-4} 
                                        & Synthesis                              & tacotron2                              & tts\_angular                 \\ \hline
\multirow{5}{*}{Other}                  & \multirow{5}{*}{-}                     & pytorch\_struct                        & moco                         \\ \cdashline{3-4} 
                                        &                                        & functorch\_dp\_cifar10                 & maml\_omniglot               \\ \cdashline{3-4} 
                                        &                                        & functorch\_maml\_omniglot              & pyhpc\_equation\_of\_state   \\ \cdashline{3-4} 
                                        &                                        & lennard\_jones                         & pyhpc\_isoneutral\_mixing    \\ \cdashline{3-4} 
                                        &                                        & pyhpc\_turbulent\_kinetic\_energy      & maml                         \\ \hline
\end{tabular}
\end{table*}

==> table_optimization.tex <==
%auto-ignore
\begin{table}[]
\centering
\scriptsize
% narrow the space between columns
\setlength{\tabcolsep}{1pt}


\caption{The impact to TFLOPS by our optimizations. This table shows the change for achieved TFLOPS and missing TFLOPS caused by idleness and data movement of the original and optimized models in Figure~\ref{fig:speedup_train}. remove original, add percentage, 
}
\label{table:optimization}

\begin{tabular}{|c|c|c|c|c|}
\hline
Model                                                                          & Execution Time  & TFLOPS         & Idleness       & Data Movement  \\ \hline
resnext50\_32x4d                                                               & 37.36(+55.0\%)  & 6.28(+35.6\%)  & 6.28(-30.9\%)  & 6.28(+0.0\%)   \\ \hline
phlippe\_densenet                                                              & 41.21(+45.0\%)  & 4.38(+30.0\%)  & 4.38(+20.3\%)  & 4.38(+0.0\%)   \\ \hline
mobilenet\_v3\_large                                                           & 41.74(+32.0\%)  & 1.78(+13.4\%)  & 1.78(-21.6\%)  & 1.78(+33.5\%)  \\ \hline
resnet18                                                                       & 13.87(+32.0\%)  & 6.87(+15.1\%)  & 6.87(-31.4\%)  & 6.87(+0.0\%)   \\ \hline
resnet152                                                                      & 118.31(+31.0\%) & 10.01(+18.3\%) & 10.01(-73.0\%) & 10.01(+0.0\%)  \\ \hline
speech\_transformer                                                            & 154.54(+30.0\%) & 5.88(+35.8\%)  & 5.88(+10.7\%)  & 5.88(+54.6\%)  \\ \hline
\begin{tabular}[c]{@{}c@{}}detectron2\_maskrcnn\_\\ r\_50\_fpn\end{tabular}    & 83.14(+26.0\%)  & 7.42(+8.0\%)   & 7.42(+2.2\%)   & 7.42(+1.4\%)   \\ \hline
dcgan                                                                          & 50.77(+20.0\%)  & 6.68(+16.4\%)  & 6.68(-9.4\%)   & 6.68(+18.9\%)  \\ \hline
\begin{tabular}[c]{@{}c@{}}detectron2\_maskrcnn\_\\ r\_101\_fpn\end{tabular}   & 111.13(+19.0\%) & 8.13(+19.2\%)  & 8.13(+19.0\%)  & 8.13(+9.2\%)   \\ \hline
hf\_BigBird                                                                    & 285.12(+14.0\%) & 7.85(+14.3\%)  & 7.85(-19.3\%)  & 7.85(+15.4\%)  \\ \hline
mnasnet1\_0                                                                    & 32.66(+14.0\%)  & 2.8(+15.7\%)   & 2.8(-30.7\%)   & 2.8(+0.0\%)    \\ \hline
\begin{tabular}[c]{@{}c@{}}timm\_vision\_\\ transformer\end{tabular}           & 31.74(+14.0\%)  & 8.72(+21.3\%)  & 8.72(+22.1\%)  & 8.72(+21.8\%)  \\ \hline
phlippe\_resnet                                                                & 11.87(+10.0\%)  & 3.97(+28.9\%)  & 3.97(+71.9\%)  & 3.97(+0.0\%)   \\ \hline
shufflenet\_v2\_x1\_0                                                          & 40.38(+10.0\%)  & 3.5(+11.5\%)   & 3.5(-39.0\%)   & 3.5(+0.0\%)    \\ \hline
\begin{tabular}[c]{@{}c@{}}pytorch\_CycleGAN\_\\ and\_pix2pix\end{tabular}     & 7655.64(+9.0\%) & 6.37(+2.7\%)   & 6.37(+7.6\%)   & 6.37(+4.2\%)   \\ \hline
timm\_efficientnet                                                             & 44.58(+9.0\%)   & 2.63(+11.9\%)  & 2.63(-27.2\%)  & 2.63(+21.3\%)  \\ \hline
functorch\_dp\_cifar10                                                         & 68.14(+8.0\%)   & 1.6(+73.9\%)   & 1.6(+99.1\%)   & 1.6(+73.6\%)   \\ \hline
opacus\_cifar10                                                                & 59.11(+8.0\%)   & 1.96(+73.5\%)  & 1.96(+99.0\%)  & 1.96(+104.6\%) \\ \hline
resnet50                                                                       & 44.14(+7.0\%)   & 9.23(+14.5\%)  & 9.23(-44.0\%)  & 9.23(+0.0\%)   \\ \hline
vision\_maskrcnn                                                               & 240.11(+7.0\%)  & 9.14(-2.9\%)   & 9.14(+10.3\%)  & 9.14(-20.5\%)  \\ \hline
densenet121                                                                    & 393.54(+6.0\%)  & 7.88(+4.4\%)   & 7.88(-87.6\%)  & 7.88(+14.3\%)  \\ \hline
timm\_efficientdet                                                             & 313.78(+6.0\%)  & 3.53(+6.3\%)   & 3.53(-28.0\%)  & 3.53(+8.5\%)   \\ \hline
\end{tabular}

\end{table}

==> table_slowdown_cudnn.tex <==
%auto-ignore
\begin{table}[]


\caption{The speedup of 17 models running with cuDNN 8.7.0 compared with cuDNN 8.3.2. The \texttt{cudnn.benchmark} has been disabled except model timm\_nfnet.}
\label{table:slowdown cudnn}
\centering



\begin{tabular}{|c|cc|}
\hline
\multirow{2}{*}{Model}             & \multicolumn{2}{c|}{Speedup}              \\ \cline{2-3} 
                                   & \multicolumn{1}{c|}{Training} & Inference \\ \hline
dcgan                              & \multicolumn{1}{c|}{1.08}     & 0.41      \\ \hline
phlippe\_resnet                    & \multicolumn{1}{c|}{1.03}     & 0.96      \\ \hline
maml\_omniglot                     & \multicolumn{1}{c|}{0.98}     & 0.97      \\ \hline
timm\_efficientdet                 & \multicolumn{1}{c|}{0.97}     & 0.99      \\ \hline
pytorch\_unet                      & \multicolumn{1}{c|}{0.96}     & 1.15      \\ \hline
detectron2\_fasterrcnn\_r\_101\_c4 & \multicolumn{1}{c|}{0.94}     & 0.95      \\ \hline
detectron2\_maskrcnn\_r\_101\_c4   & \multicolumn{1}{c|}{0.94}     & 0.95      \\ \hline
detectron2\_maskrcnn\_r\_50\_c4    & \multicolumn{1}{c|}{0.93}     & 0.95      \\ \hline
timm\_regnet                       & \multicolumn{1}{c|}{0.93}     & 1         \\ \hline
detectron2\_fasterrcnn\_r\_50\_c4  & \multicolumn{1}{c|}{0.92}     & 0.95      \\ \hline
timm\_nfnet                        & \multicolumn{1}{c|}{0.92}     & 1         \\ \hline
timm\_resnest                      & \multicolumn{1}{c|}{0.92}     & 1         \\ \hline
functorch\_maml\_omniglot          & \multicolumn{1}{c|}{0.89}     & 0.96      \\ \hline
\end{tabular}
\end{table}
